Canonical tessellations of decorated hyperbolic surfaces

A decoration of a hyperbolic surface of finite type is a choice of circle, horocycle or hypercycle about each cone-point, cusp or flare of the surface, respectively. In this article we show that a decoration induces a unique canonical tessellation and dual decomposition of the underlying surface. They are analogues of the weighted Delaunay tessellation and Voronoi decomposition in the Euclidean plane. We develop a characterisation in terms of the hyperbolic geometric equivalents of Delaunay's empty-discs and Laguerre's tangent-distance, also known as power-distance. Furthermore, the relation between the tessellations and convex hulls in Minkowski space is presented, generalising the Epstein-Penner convex hull construction. This relation allows us to extend Weeks' flip algorithm to the case of decorated finite type hyperbolic surfaces. Finally, we give a simple description of the configuration space of decorations and show that any fixed hyperbolic surface only admits a finite number of combinatorially different canonical tessellations.

==> references.tex <==
\bib{Akiyoshi00}{article}{
   title={Finiteness of Polyhedral Decompositions of Cusped Hyperbolic
      Manifolds Obtained by the Epstein-Penner's Method},
   author={Akiyoshi, Hirotaka},
   journal={Proc. Amer. Math. Soc.},
   volume={129},
   number={8},
   pages={2431--2439},
   date={2000}
}
\bib{Beardon83}{book}{
   title={The Geometry of Discrete Groups},
   author={Beardon, Alan F.},
   publisher={Springer},
   place={New York, USA},
   date={1983},
   series={GTM},
   volume={91}
}
\bib{Benz73}{book}{
   title={Vorlesungen \"uber die Geometrie der Algebren},
   author={Benz, Walter},
   publisher={Springer},
   place={Berlin, Germany},
   date={1973},
   series={Grundlehren math. Wiss.},
   volume={197}
}
\bib{Blaschke29}{book}{
   title={Vorlesungen über Differentialgeometrie und geometrische Grundlagen
      von Einsteins Relativitätstheorie. III. Differentialgeometrie der Kreise und
      Kugeln},
   author={Blaschke, Wilhelm},
   publisher={Springer},
   place={Berlin, Germany},
   date={1929},
   series={Grundlehren math. Wiss.},
   volume={29}
}
\bib{BobenkoEtAl21}{book}{
   title={Non-Euclidean Laguerre Geometry and Incircular Nets},
   author={Bobenko, Alexander I.},
   author={Lutz, Carl O. R.},
   author={Pottmann, Helmut},
   author={Techter, Jan},
   publisher={Springer},
   place={Cham, Switzerland},
   date={2021},
   series={SpringerBriefs in Mathematics}
}
\bib{BobenkoEtAl15}{article}{
   title={Discrete conformal maps and ideal hyperbolic polyhedra},
   author={Bobenko, Alexander I.},
   author={Pinkall, Ulrich},
   author={Springborn, Boris},
   journal={Geom. Topol.},
   volume={19},
   number={4},
   date={2015},
   pages={2155--2215}
}
\bib{BobenkoSpringborn07}{article}{
   title={A discrete Laplace-Beltrami operator for simplicial surfaces},
   author={Bobenko, Alexander I.},
   author={Springborn, Boris},
   journal={Discrete Comput. Geom.},
   volume={38},
   number={4},
   date={2007},
   pages={740--756}
}
\bib{BogdanovEtAl14}{article}{
   title={Hyperbolic Delaunay Complexes and Voronoi Diagrams Made Practical},
   author={Bogdanov, Mikhail}
   author={Devillers, Olivier}
   author={Teillaud, Monique},
   journal={J. Comput. Geom.},
   volume={5},
   number={1},
   date={2014},
   pages={56--85},
}
\bib{BowditchEpstein88}{article}{
   title={Natural triangulations associated to a surface},
   author={Bowditch, Brian H.},
   author={Epstein, David B. A.},
   journal={Topology},
   volume={27},
   date={1988},
   pages={91--117}
}
\bib{BridsonHaefliger99}{book}{
   title={Metric Spaces of Non-Positive Curvature},
   author={Bridson, Martin R.},
   author={Haefliger, Andr{\'e}},
   series={Grundlehren Math. Wiss.},
   volume={319},
   publisher={Springer},
   place={Berlin, Germany},
   date={1999}
}
\bib{CannonEtAl97}{article}{
   title={Hyperbolic Geometry},
   author={Cannon, James W.},
   author={Floyd, William J.},
   author={Kenyon, Richard},
   author={Parry, Walter},
   booktitle={Flavors of Geometry},
   series={MSRI Publications},
   volume={31},
   publisher={Cambridge University Press},
   date={1997}
}
\bib{Cecil92}{book}{
   title={Lie sphere geometry: with applications to submanifolds},
   author={Cecil, Thomas E.},
   series={Universitext},
   publisher={Springer},
   place={New York, USA},
   date={1992}
}
\bib{CooperEtAl00}{book}{
   title={Three-dimensional orbifolds and cone-manifolds},
   author={Cooper, Daryl},
   author={Hodgson, Craig D.},
   author={Kerckhoff, Steve},
   series={MSJ memoirs},
   volume={5},
   date={2000},
   publisher={Math. Soc. Japan},
   place={Tokyo, Japan}
}
\bib{CooperLong13}{article}{
   title={A generalization of the Epstein-Penner construction to projective
      manifolds},
   author={Cooper, Daryl},
   author={Long, Darren},
   journal={Proc. Amer. Math. Soc.},
   volume={143},
   number={10},
   date={2013},
   pages={4561--4569}
}
\bib{DeLoeraEtAl10}{book}{
   title={Triangulations},
   author={{De L}oera, Jes{\'u}s A.},
   author={Rambau, J{\"o}rg},
   author={Santos, Francisco},
   series={Algo. Comput. Math.},
   volume={25},
   publisher={Springer},
   place={Berlin},
   date={2010}
}
\bib{Delaunay34}{article}{
   title={Sur la sph{\`e}re vide},
   author={Delaunay, Boris},
   journal={Bull. Acad. Sci URSS, VII. Ser.},
   number={6},
   date={1934},
   pages={793--800},
}
\bib{DespreEtAl20}{article}{
   title={Flipping geometric triangulations on hyperbolic surfaces},
   author={Despr{\'e}, Vincent},
   author={Schlenker, Jean-Marc},
   author={Teillaud, Monique},
   editor={Cabello, Sergio},
   editor={Chen, Danny Z.},
   booktitle={36th International Symposium on Computational Geometry (SoCG 2020)},
   series={Leibniz International Proceedings in Informatics (LIPIcs)},
   publisher={Schloss Dagstuhl -- Leibniz-Zentrum f{\"u}r Informatik},
   address={Dagstuhl, Germany},
   volume={164},
   date={2020},
   pages={35:1--35:16}
}
\bib{Dirichlet50}{article}{
   title={\"Uber die Reduction der positiven quadratischen Formen mit drei unbestimmten
      ganzen Zahlen},
   author={Dirichlet, G. Lejeune},
   journal={J. Reine Angew. Math.},
   volume={40},
   date={1850},
   pages={209--227}
}
\bib{Edelsbrunner00}{article}{
   title={Triangulations and meshes in computational geometry},
   author={Edelsbrunner, Herbert},
   journal={Acta Numerica},
   volume={9},
   date={2000},
   pages={133--213}
}
\bib{EpsteinPenner88}{article}{
   title={Euclidean decompositions of noncompact hyperbolic manifolds},
   author={Epstein, David B. A.},
   author={Penner, Robert C.},
   journal={J. Differential Geom.},
   volume={27},
   number={1},
   date={1988},
   pages={67--80}
}
\bib{EricksonLin21}{article}{
   title={A toroidal Maxwell–Cremona–Delaunay Correspondence},
   author={Erickson, Jeff},
   author={Lin, Patrick},
   journal={J. Comput. Geom.},
   volume={12},
   number={2},
   date={2021},
   pages={55--85}
}
\bib{Fillastre08}{article}{
   title={Polyhedral hyperbolic metrics on surfaces},
   author={Fillastre, Fran{\c{c}}ois},
   journal={Geom. Dedicata},
   volume={134},
   number={1},
   date={2008},
   pages={177--196},
}
\bib{Fillastre13}{article}{
   title={Fuchsian convex bodies: basics of Brunn-Minkowski theory},
   author={Fillastre, Fran{\c{c}}ois},
   journal={Geom. Funct. Anal.},
   volume={23},
   date={2013},
   pages={295--333},
}
\bib{GelfandEtAl94}{book}{
   title={Discriminants, Resultants, and Multidimensional Determinants},
   author={Gelfand, Israel M.},
   author={Kapranov, Mikhail M.},
   author={Zelevinsky, Andrei V.},
   publisher={Birkh{\"a}user},
   place={Boston, MA},
   date={1994}
}
\bib{GillespieEtAl21}{article}{
   title={Discrete conformal equivalence of polyhedral surfaces},
   author={Gillespie, Mark},
   author={Springborn, Boris},
   author={Crane, Keenan},
   journal={ACM Trans. Graph.},
   volume={40},
   number={4},
   date={2021},
   pages={1--20}
}
\bib{GuEtAl18a}{article}{
   title={A discrete uniformization theorem for polyhedral surfaces},
   author={Gu, Xianfeng},
   author={Luo, Feng},
   author={Sun, Jian},
   author={Wu, Tianqi},
   journal={J. Differential Geom.},
   volume={109},
   number={2},
   date={2018},
   pages={223--256},
}
\bib{GuEtAl18b}{article}{
   title={A discrete uniformization theorem for polyhedral surfaces II},
   author={Gu, Xianfeng},
   author={Guo, Ren},
   author={Luo, Feng},
   author={Sun, Jian},
   author={Wu, Tianqi},
   journal={J. Differential Geom.},
   volume={109},
   number={3},
   date={2018},
   pages={431--466},
}
\bib{Harer88}{article}{
   title={The Cohomology of the Moduli Space of Curves},
   author={Harer, John L.},
   editor={Sernesi, Edoardo},
   booktitle={Theory of moduli},
   series={Lecture notes in mathematics},
   publisher={Springer},
   address={Berlin, Germany},
   volume={1337},
   date={1988},
   pages={138--221}
}
\bib{ImaiEtAl85}{article}{
   title={Voronoi Diagram in the Laguerre Geometry and its Applications},
   author={Imai, Hiroshi},
   author={Iri, Masao},
   author={Murota, Kazuo},
   journal={SIAM J. Comput.},
   volume={14},
   number={1},
   date={1985},
   pages={93--105}
}
\bib{IndermitteEtAl01}{article}{
   title={Voronoi diagrams on piecewise flat surfaces and an application to
      biological growth},
   author={Indermitte, Claude},
   author={Liebling, Thomas M.},
   author={Troyanov, Marc},
   author={Clemencon, Heinz},
   journal={Theor. Comput. Sci.},
   volume={263},
   number={1-2},
   date={2001},
   pages={263--274}
}
\bib{Izmestiev19}{article}{
   title={Statics and kinematics of frameworks in Euclidean and non-Euclidean geometry},
   booktitle={Eighteen Essays in Non-Euclidean Geometry},
   author={Izmestiev, Ivan},
   editor={Alberge, Vincent},
   editor={Papadopoulos, Athanase},
   series={IRMA lectures in mathematics and theoretical physics},
   number={29},
   publisher={EMS Publishing},
   date={2019},
   pages={191--233}
}
\bib{JoswigEtAl20}{article}{
   title={Secondary fans and secondary polyhedra of punctured Riemann surfaces},
   author={Joswig, Michael},
   author={L{\"o}we, Robert},
   author={Springborn, Boris},
   journal={Exp. Math.},
   volume={29},
   number={4},
   date={2020},
   pages={426--442}
}
\bib{Leibon02}{article}{
   title={Characterizing the Delaunay decompositions of compact hyperbolic surfaces},
   author={Leibon, Gregory},
   journal={Geom. Topol.},
   volume={6},
   number={1},
   date={2002},
   pages={361--391}
}
\bib{NaatanenPenner91}{article}{
   title={The Convex Hull Construction for Compact Surfaces
      and the Dirichlet Polygon},
   author={N{\"a}{\"a}t{\"a}nen, Marjatta},
   author={Penner, Robert C.},
   journal={Bull. Lond. Math. Soc.},
   volume={23},
   number={6},
   date={1991},
   pages={568--574}
}
\bib{Penner87}{article}{
   title={The Decorated Teichm{\"u}ller Space of Punctured Surfaces},
   author={Penner, Robert C.},
   journal={Commun. Math. Phys.},
   number={113},
   date={1987},
   pages={299--339}
}
\bib{Penner12}{book}{
   title={Decorated Teichm{\"u}ller Theory},
   author={Penner, Robert C.},
   publisher={EMS},
   address={Z{\"u}rich, Switzerland},
   date={2012}
}
\bib{Poincare82}{article}{
   title={Th{\'e}orie des groupes fuchsiens},
   author={Poincar{\'e}, Henri},
   journal={Acta Math.},
   volume={1},
   date={1882},
   pages={1--62}
}
\bib{Prosanov20}{article}{
   title={Ideal polyhedral surfaces in Fuchsian manifolds},
   author={Prosanov, Roman},
   journal={Geom. Dedicata},
   volume={206},
   date={2020},
   pages={151--179},
}
\bib{Ratcliffe94}{book}{
   title={Foundations of Hyperbolic Manifolds},
   author={Ratcliffe, John G.},
   publisher={Springer},
   address={New York},
   date={1994}
   series={GTM},
   volume={149}
}
\bib{Rivin94}{article}{
   title={Euclidean structures on simplicial surfaces and hyperbolic volume},
   author={Rivin, Igor},
   journal={Ann. Math.},
   volume={139},
   number={3},
   date={1994},
   pages={553--580}
}
\bib{SakumaWeeks95}{article}{
   title={The generalized tilt formula},
   author={Sakuma, Makoto},
   author={Weeks, Jeffrey R.},
   journal={Geom. Dedicata},
   volume={55},
   number={2},
   date={1995},
   pages={115--123}
}
\bib{Springborn08}{article}{
   title={A variational principle for weighted Delaunay triangulations
      and hyperideal polyhedra},
   author={Springborn, Boris},
   journal={J. Diff. Geom.},
   volume={78},
   number={2},
   date={2008},
   pages={333-367}
}
\bib{Springborn20}{article}{
   title={Ideal Hyperbolic Polyhedra and Discrete Uniformization},
   author={Springborn, Boris},
   journal={Discrete Comput. Geom.},
   volume={64},
   date={2020},
   pages={63--108}
}
\bib{Thurston97}{book}{
   title={Three-Dimensional geometry and topology},
   author={Thurston, William P.},
   editor={Levy, Silvio},
   publisher={Princeton University Press},
   place={Princeton, NJ},
   date={1997},
   series={Princeton mathematical series},
   volume={35}
}
\bib{TillmannWong16}{article}{
   title={An algorithm for the Euclidean cell decomposition of a cusped
      strictly convex projective surface},
   author={Tillmann, Stephan},
   author={Wong, Sampson},
   journal={J. Comput. Geom.},
   volume={7},
   number={1},
   date={2016},
   pages={237--255}
}
\bib{Ushijima99}{article}{
   title={A Canonical Cellular Decomposition of the Teichm{\"u}ller Space
      of Compact Surfaces with Boundary},
   author={Ushijima, Akira},
   journal={Commun. Math. Phy.},
   volume={201},
   number={2},
   date={1999},
   pages={305--326}
}
\bib{Ushijima02}{article}{
   title={The Tilt Formula for Generalized Simplices in Hyperbolic Space},
   author={Ushijima, Akira},
   journal={Discrete Comput. Geom.},
   volume={28},
   number={1},
   date={2002},
   pages={19--27},
}
\bib{Voronoi08}{article}{
   title={Nouvelles applications des param{\`e}tres continues {\`a} la
      th{\'e}orie des formes quadratiques, II},
   subtitle={Recherches sur les parall{\'e}lo{\'e}dres primitifs},
   author={Vorono{\"{\i}}, Georges F.},
   journal={J. Reine Angew. Math.},
   volume={134},
   date={1908},
   pages={198--287}
}
\bib{Weeks93}{article}{
   title={Convex hulls and isometries of cusped hyperbolic 3-manifolds},
   author={Weeks, Jeffrey R.},
   journal={Topology Appl.},
   volume={52},
   number={2},
   date={1993},
   pages={127--149}
}
\bib{Yaglom68}{book}{
   title={Complex numbers in geometry},
   author={Yaglom, Isaak M.},
   publisher={Academic Press},
   address={New York, USA},
   date={1968}
}

